A novel measurement of marginal Alfv\'{e}n Eigenmode stability during high power auxiliary heating in JET

The interaction of Alfv\'{e}n Eigenmodes (AEs) and energetic particles is one of many important factors determining the success of future tokamaks. In JET, eight in-vessel antennas were installed to actively probe stable AEs with frequencies ranging 25-250 kHz and toroidal mode numbers $\vert n \vert < 20$. During the 2019-2020 deuterium campaign, almost 7500 resonances and their frequencies $f_0$, net damping rates $\gamma < 0$, and toroidal mode numbers were measured in almost 800 plasma discharges. From a statistical analysis of this database, continuum and radiative damping are inferred to increase with edge safety factor, edge magnetic shear, and when including non-ideal effects. Both stable AE observations and their associated damping rates are found to decrease with $\vert n \vert$. Active antenna excitation is also found to be ineffective in H-mode as opposed to L-mode; this is likely due to the increased edge density gradient's effect on accessibility and ELM-related noise's impact on mode identification. A novel measurement is reported of a marginally stable, edge-localized Ellipticity-induced AE probed by the antennas during high-power auxiliary heating (ICRH and NBI) up to 25 MW. NOVA-K kinetic-MHD simulations show good agreement with experimental measurements of $f_0$, $\gamma$, and $n$, indicating the dominance of continuum and electron Landau damping in this case. Similar experimental and computational studies are planned for the recent hydrogen and ongoing tritium campaigns, in preparation for the upcoming DT campaign.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

    \yk{
    The \Alfven continua for this pulse (see \cref{fig:novak_both}) exhibit an interesting feature: the \TAE and \EAE gaps exist at the \emph{same} frequency but over different radial ranges - core and edge, respectively - due to the differential plasma rotation (see \cref{fig:profiles}) and associated Doppler shift. Though not shown here, this result is confirmed with the \Alfven continuum solver \CSCAS \cite{cscas_huysmans2001} using the magnetic geometry output from \HELENA \cite{helena_huysmans1991}. Therefore, it is reasonable to ask whether the \AEAD is resonating with an edge \EAE instead of a core \TAE.
    }
    
    \yk{
    A scan in the $\q$ profile - i.e. a translation up/down by $\pm0.1$ and $\pm0.2$ - in \NOVAK finds \emph{no} $\n=3$ or $5$ eigenmode solutions in the \TAE gap close to the experimentally measured frequency. Importantly, the $n=5$ \EAE is the most robust solution to this sensitivity study. However, by drastically lowering the shear (so that $\qnf \approx 2$), an $\n=3$ \TAE solution appears near $\sqrt{\psin}\approx 0.4$ with frequency $\fo \approx \SI{235}{kHz}$. This implies that it may be possible to adjust plasma profiles to find a \TAE located in the core/mid-radius, but such profiles are outside of experimental uncertainties, and we conclude that our measurement corresponds to the edge-localized \EAE predicted by the most reasonable assumptions.
    }
    
    \yk{
    Yet pursuing such \TAE solutions is not without some experimental motivation: the pulse of interest in this paper, JPN~94703, is very similar to another plasma discharge, JPN~95683, which was also part of JET's three-ion D-DNBI-$\Hethree$ heating scenario experiments with $\nHethree/\ne \approx 18\%-22\%$. Although not shown here, global magnetic parameters and their time evolutions are almost identical; however, JPN~95863 had less \NBI but more \ICRH power: $\Pnbi \approx \SI{18.5}{MW}$ and $\Picrh \approx \SI{5.5}{MW}$. This resulted in a lower central density but higher core temperature: $\neo \approx \SI{6\times10^{19}}{m^{-3}}$ and $\Teo \approx \SI{6}{keV}$.
    }
    
    \yk{
    The additional \ICRH in JPN~95683 \emph{destabilized} \TAEs with toroidal mode numbers $\n = 2,3,4$ and lab-frame frequencies $\fo \approx \SI{185,205,225}{kHz}$, respectively. Soft X-ray, interferometry, and reflectometry indicate that these \TAEs are localized at mid-radius around $R \approx \SI{3.3-3.4}{m}$ ($\sqrt{\psin} \approx 0.35-0.50$), with $\Ro \approx \SI{3}{m}$. It was hoped that the \AEAD measured the associated stable $\n=5$ \TAE in JPN~94703, yet the computational analyses of this and the previous section show that this is unlikely. Further analysis of JPN~95683 should be pursued, but is beyond the scope of the present work.
    }
